Bayesian Nonparametric Multilevel Clustering with Group-Level Contexts

We present a Bayesian nonparametric framework for multilevel clustering which utilizes group-level context information to simultaneously discover low-dimensional structures of the group contents and partitions groups into clusters. Using the Dirichlet process as the building block, our model constructs a product base-measure with a nested structure to accommodate content and context observations at multiple levels. The proposed model possesses properties that link the nested Dirichlet processes (nDP) and the Dirichlet process mixture models (DPM) in an interesting way: integrating out all contents results in the DPM over contexts, whereas integrating out group-specific contexts results in the nDP mixture over content variables. We provide a Polya-urn view of the model and an efficient collapsed Gibbs inference procedure. Extensive experiments on real-world datasets demonstrate the advantage of utilizing context information via our model in both text and image domains.

==> framework5__Dinh_Phung_s_conflicted_copy_2014-01-19_.tex <==

\subsection{Model description and stick-breaking}

Consider data presented in a two-level group structure as follows.
Denote by $J$ the number of groups; each group $j$ contains $N_{j}$
exchangeable data points, represented by $\bw_{j}=\left\{ w_{j1},w_{j2},\ldots,w_{jN_{j}}\right\} $.
For each group $j$, the group-specific context data is denoted by
$x_{j}$. Assuming that the groups are exchangeable, the overall data
is $\left\{ (x_{j},\bw_{j})\right\} _{j=1}^{J}$. The collection $\left\{ \bw_{1},\ldots,\bw_{J}\right\} $
represents observations of the group contents, and $\left\{ x_{1},\ldots,x_{J}\right\} $
represents observations of the group-level contexts.

We now describe the generative process of \modelname ~that generates
a two-level clustering of this data. We use a group-level DP mixture
to generate an infinite cluster model for groups. Each group cluster
$k$ is associated with an atom having the form of a pair $(\phi_{k},Q_{k}^{*})$
where $\phi_{k}$ is a parameter that generates the group-level contexts
within the cluster and $Q_{k}^{*}$ is a measure that generates the
group contents within the same cluster. 

To generate atomic pairs of context parameter and measure-valued content
parameter, we introduce a product base-measure of the form $H\times\DP(vQ_{0})$
for the group-level DP mixture. Drawing from a DP mixture with this
base measure, each realization is a pair $(\theta_{j},Q_{j})$; $\theta_{j}$
is then used to generate the context $x_{j}$ and $Q_{j}$ is used
to repeatedly produce the set of content observations $w_{ji}$ within
the group $j$. Specifically,
\begin{align}
U\sim\dirproc\left(\alpha(H\times\DP(vQ_{0}))\right) & \,\text{where }Q_{0}\sim\dirproc\left(\eta S\right)\nonumber \\
(\theta_{j},Q_{j})\iid U & \ \text{for each group\ }j\label{eq:MC2}\\
x_{j}\sim F(.\vert\theta_{j}),\quad\varphi_{ji} & \iid Q_{j},\quad w_{ji}\sim Y\left(.\vert\varphi_{ji}\right)\nonumber 
\end{align}
In the above, $H$ and $S$ are respectively base measures for context
and content parameters $\theta_{j}$ and $\varphi_{ji}$. The context
and content observations are then generated via the likelihood kernels
$F\left(\cdot\gv\theta_{j}\right)$ and $Y\left(\cdot\gv\varphi_{ji}\right)$.
To simplify inference, $H$ and $S$ are assumed to be conjugate to
$F$ and $Y$ respectively. The generative process is illustrated
in Figure \ref{fig:J3}.

\begin{figure}
\begin{centering}
\includegraphics[scale=0.25]{WSNDP}\vspace{-0.1in}

\par\end{centering}

\caption{Graphical model representation for the proposed model. Right figure
illustrates a stick breaking representation.\label{fig:J3}}
\end{figure}



\subsubsection*{Stick-breaking representation}

We now derive the stick-breaking construction for \modelname$\ $
$\ $where all the random discrete measures are specified by a distribution
over integers and a countable set of atoms. The random measure $U$
in Eq. (\ref{eq:MC2}) has the stick-breaking form:\vspace{-0.05in}
\begin{align}
U & =\sum_{k=1}^{\infty}\pi_{k}\delta_{\left(\phi_{k},Q_{k}^{*}\right)}\label{eq:}
\end{align}
where $\pi\sim\gempdf\left(\alpha\right)$ and $\left(\phi_{k},Q_{k}^{*}\right)\iid H\times\dirproc\left(vQ_{0}\right)$.
Equivalently, this means $\phi_{k}$ is drawn i.i.d. from $H$ and
$Q_{k}^{*}$ drawn i.i.d. from $\dirproc\left(vQ_{0}\right)$. Since
$Q_{0}\sim\dirproc\left(\eta S\right)$, $Q_{0}$ and $Q_{k}^{*}$
have the standard HDP \cite{Teh_etal_06hierarchical} stick-breaking
forms: $Q_{0}=\sum_{m=1}^{\infty}\epsilon_{m}\delta_{\psi_{m}}$where
$\bepsilon\sim\textrm{GEM}(\eta)$, $\psi_{m}\iid S$; $Q_{k}^{*}=\sum_{m=1}^{\infty}\tau_{k,m}\delta_{\psi_{m}}$
where $\btau_{k}=\left(\tau_{k1},\tau_{k2},\ldots\right)\sim\dirproc\left(v,\bepsilon\right)$.

For each group $j$ we sample the parameter pair $\left(\theta_{j},Q_{j}\right)\iid U$;
equivalently, this means drawing $z_{j}\iid\pi$ and letting $\theta_{j}=\phi_{z_{j}}$
and $Q_{j}=Q_{z_{j}}^{*}$. For the $i$-th content data within the
group $j$, the content parameter $\varphi_{ji}$ is drawn $\iid Q_{j}=Q_{z_{j}}^{*}$;
equivalently, this means drawing $l_{ji}\iid\tau_{z_{j}}$ and letting
$\varphi_{ji}=\psi_{l_{ji}}$. Figure \ref{fig:J3} presents the graphical
model of this stick-breaking representation.


\subsection{Inference and Polya Urn View}

We use collapsed Gibbs sampling, integrating out $\phi_{k}$(s), $\psi_{m}$(s),
$\pi$ and $\tau_{k}$ (s). Latent variables $\bz$, $\bl$, $\bepsilon$
and the hyper-parameters $\alpha$, $v$, $\eta$ will be resampled.
We only describe the key inference steps in sampling $\bz,\bl$ and
$\bepsilon$ here and refer to Appendix \ref{sub:Model-Inference-Derivations}
for the rest of the details (including how to sample the hyper-parameters).


\textbf{Sampling} $\bz$. The required conditional distribution is
$p(z_{j}=k\gv\bz_{-j},\bl,\bx,\alpha,H)\propto$
\begin{align*}
 & p\left(z_{j}=k|\bz_{-j},\alpha\right)p\left(x_{j}|z_{j}=k,\bz_{-j},\bx_{-j},H\right)\\
 & \times p\left(l_{j*}|z_{j}=k,\bl_{-j*},\bz_{-j},\bepsilon,v\right)
\end{align*}
The first term can be recognized as a form of the Chinese restaurant
process (CRP). The second term is the predictive likelihood for the
context observations under the component $\phi_{k}$ after integrating
out $\phi_{k}$. This can be evaluated analytically due to conjugacy
of $F$ and $H$. The last term is the predictive likelihood for the
group content-index $l_{j*}=\left\{ l_{ji}\vert i=1\ldots N_{j}\right\} $.
Since $l_{ji}\gv z_{j}=k\iid\multpdf\left(\btau_{k}\right)$ where
$\btau_{k}\sim\dirpdf\left(v\epsilon_{1},\ldots,v\epsilon_{M},\epsilon_{\text{new}}\right)$,
the last term can also be evaluated analytically by integrating out
$\btau_{k}$ using the Multinomial-Dirichlet conjugacy property.

\textbf{Sampling} $\bl$. Let $w_{-ji}$ be the same set as $\bw$
excluding $w_{ji}$, let $w_{-ji}(m)=\left\{ w_{j'i'}\vert(j'i')\neq(ji)\wedge l_{j'i'}=m\right\} $
and $\bl_{-ij}(k)=\left\{ l_{j'i'}\vert(j'i')\neq(ji)\wedge z_{j'}=k\right\} $.
Then $p\left(l_{ji}=m\mid l_{-ji},z_{j}=k,z_{-j},v,\bw,\bepsilon,S\right)\propto$
\begin{align*}
 & p(w_{ji}\vert\bl,w_{-ji},S)\ p(l_{ji}=m\vert\bl_{-ji},z_{j}=k,z_{-j},\bepsilon,v)\\
= & p\left(w_{ji}\mid w_{-ji}(m),S\right)p\left(l_{ji}=m\mid\bl_{-ji}(k),\bepsilon,v\right)
\end{align*}


The first term is the predictive likelihood under mixture component
$\psi_{m}$ after integrating out $\psi_{m}$, which can be evaluated
analytically due to the conjugacy of $Y$ and $S$. The second term
is in the form of a CRP similar to the one that arises during inference
for HDP \cite{Teh_etal_06hierarchical}. 

\textbf{Sampling} $\bepsilon$. Sampling $\bepsilon$ requires information
from both $\bz$ and $\bl$.
\begin{align}
p\left(\epsilon\mid\bl,\bz,v,\eta\right) & \propto p\left(\bl\mid\bepsilon,v,\bz,\eta\right)\times p\left(\bepsilon\mid\eta\right)\label{eq:sampling epsilon-1-1}
\end{align}
Using a similar strategy in HDP, we introduce auxiliary variables
$\left(o_{km}\right)$, then alternatively sample together with $\bepsilon$:
\begin{align*}
p\left(o_{km}=h\gv\cdot\right) & \propto\textrm{Stirl}\left(h,n_{km}\right)(v\epsilon_{m})^{h},\, h=0,1,\ldots,n_{km}\\
p\left(\bepsilon\mid\cdot\right) & \propto\epsilon_{\textrm{new}}^{\eta-1}\prod_{m=1}^{M}\epsilon_{m}^{\sum_{k}o_{km}-1}
\end{align*}
where $\textrm{Stirl}\left(h,n_{km}\right)$ is the Stirling number
of the first kind, $n_{km}$ is the count of seeing the pair $\left(z_{j}=k,l_{ji}=m\right):\forall i,j$,
and finally $M$ is the current number of active content topics. It
clear that $o_{km}$ can be sampled from a Multinomial distribution
and $\epsilon$ from an $\left(M+1\right)$-dim Dirichlet distribution.


\subsubsection*{Polya Urn View}

Our model exhibits a Polya-urn view using the analogy of a fleet of
buses, driving customers to restaurants. Each bus represents a group
and customers on the bus are data points within the group. For each
bus $j$, $z_{j}$ acts as the index to the restaurant for its destination.
Thus, buses form clusters at their destination restaurants according
to a CRP: a new bus drives to an existing restaurant with the probability
proportional to the number of other buses that have arrived at that
restaurant, and with probability proportional to $\alpha$, it goes
to a completely new restaurant. 

Once all the buses have delivered customers to the restaurants, \emph{all
customers at the restaurants start to behave in the same manner as
in a Chinese restaurant franchise (CRF) process}: customers are assigned
tables according to a restaurant-specific CRP; tables are assigned
with dishes $\psi_{m}$ (representing the content topic atoms) according
to a global franchise CRP. In addition to the usual CRF, at restaurant
$k$, a single dessert $\phi_{k}$ (which represents the context-generating
atom, drawing $\iid$ from $H$) will be served to all the customers
at that restaurant. Thus, every customer\emph{ }on the same bus\emph{
$j$ }will be served the same\emph{ }dessert \emph{$\phi_{z_{j}}$}.
We observe three sub-CRPs, corresponding to the three DP(s) in our
model: the CRP at the dish level is due to the $\dirproc\left(\eta S\right)$,
the CRP forming tables inside each restaurant is due to the $\DP(vQ_{0})$,
and the CRP aggregating buses to restaurants is due to the $\dirproc\left(\alpha(H\times\DP(vQ_{0}))\right)$.


\subsection{Marginalization property}

We study marginalization property for our model when either the content
topics $\varphi_{ji}$ (s) or context topics $\theta_{j}$ (s) are
marginalized out. Our main result is established in Theorem \ref{proof_Theorem4}
where we show an interesting link to nested DP and DPM via our model.

Let $H$ be a measure over some measurable spaces $(\Theta,\Sigma)$.
Let $\mathbb{P}$ be the set of all measures over $(\Theta,\Sigma)$,
suitably endowed with some $\sigma$-algebra. Let $G\sim\DP(\alpha H)$
and $\theta_{i}\iid G$. The collection $(\theta_{i})$ then follows
the DP mixture distribution which is defined formally below.
\begin{defn}
(DPM)\label{def:DPM} A DPM is a probability measure over $\Theta^{n}\ni\left(\theta_{1},\ldots,\theta_{n}\right)$
with the usual product sigma algebra $\Sigma^{n}$ such that for every
collection of measurable sets $\left\{ \left(S_{1},\ldots,S_{n}\right):S_{i}\in\Sigma,i=1,\ldots,n\right\} $:
\begin{align*}
 & \DPM(\theta_{1}\in S_{1},\ldots,\theta_{n}\in S_{n}\vert\alpha,H)\\
 & \qquad=\int\prod_{i=1}^{n}G\left(S_{i}\right)\DP\left(dG\gv\alpha H\right)
\end{align*}
\vspace{-0.2in}

\end{defn}
We now state a result regarding marginalization of draws from a DP
mixture with a joint base measure. Consider two measurable spaces
$(\Theta_{1},\Sigma_{1})$ and $(\Theta_{2},\Sigma_{2})$ and let
$(\Theta,\Sigma)$ be their product space where $\Theta=\Theta_{1}\times\Theta_{2}$
and $\Sigma=\Sigma_{1}\times\Sigma_{2}$. Let $H^{*}$ be a measure
over the product space $\Theta=\Theta_{1}\times\Theta_{2}$ and let
$H_{1}$ be the marginal of $H^{*}$ over $\Theta_{1}$ in the sense
that for any measurable set $A\in\Sigma_{1}$, $H_{1}\left(A\right)=H^{*}\left(A\times\Theta_{2}\right)$.
Then drawing $(\theta_{i}^{(1)},\theta_{i}^{(2)})$ from a DP mixture
with base measure $\alpha H$ and marginalizing out $(\theta_{i}^{(2)})$
is the same as drawing $(\theta_{i}^{(1)})$ from a DP mixture with
base measure $H_{1}$. Formally
\begin{prop}
\label{thm:marginalization_theorem}Denote by $\theta_{i}$ the pair
\textup{$\left(\theta_{i}^{\left(1\right)},\theta_{i}^{\left(2\right)}\right)$,
there holds} 
\begin{align*}
 & \DPM\left(\theta_{1}^{\left(1\right)}\in S_{1},\ldots,\theta_{n}^{\left(1\right)}\in S_{n}\gv\alpha H_{1}\right)\\
 & \quad=\DPM\left(\theta_{1}\in S_{1}\times\Theta_{2},\ldots,\theta_{n}\in S_{n}\times\Theta_{2}\gv\alpha H^{*}\right)
\end{align*}
for every collection of measurable sets $\left\{ \left(S_{1},\ldots,S_{n}\right):S_{i}\in\Sigma_{1},i=1,\ldots,n\right\} $. \end{prop}
\begin{proof}
see Appendix \ref{Proof_Prop2}.
\end{proof}
Next we give a formal definition for the nDP mixture: $\varphi_{ji}\iid Q_{j}$,
$Q_{j}\iid U$, $U\sim\DP(\alpha\DP(vQ_{0}))$, $Q_{0}\sim DP(\eta S)$.
\begin{defn}
\label{def:nDPM}(nested DP Mixture) An $\nDPM$ is a probability
measure over $\Theta^{\sum_{j=1}^{J}N_{j}}\ni\left(\varphi_{11},\ldots,\varphi_{1N_{1}},\ldots,\varphi_{JN_{J}}\right)$
equipped with the usual product sigma algebra $\Sigma^{N_{1}}\times\ldots\times\Sigma^{N_{J}}$
such that for every collection of measurable sets $\left\{ \left(S_{ji}\right):S_{ji}\in\Sigma,j=1,\ldots,J,\, i=1\ldots,N_{j}\right\} $:
\begin{align*}
 & \nDPM(\varphi_{ji}\in S_{ji},\forall i,j\vert\alpha,v,\eta,S)\\
 & \,\,\,\,=\int\int\left\{ \prod_{j=1}^{J}\int\prod_{i=1}^{N_{j}}Q_{j}\left(S_{ji}\right)U\left(dQ_{j}\right)\right\} \\
 & \,\,\,\,\,\,\,\,\,\times\DP\left(dU\gv\alpha\DP\left(vQ_{0}\right)\right)\DP\left(dQ_{0}\gv\eta,S\right)
\end{align*}


We now have the sufficient formalism to state the marginalization
result for our model.\end{defn}
\begin{thm}
\label{prop:main}Given $\alpha,H$ and $\alpha,v,\eta,S$, let $\btheta=\left(\theta_{j}:\forall j\right)$
and $\bvarphi=\left(\varphi_{ji}:\forall j,i\right)$ be generated
as in Eq (\ref{eq:MC2}). Then, marginalizing out $\bvarphi$ results
in $\DPM\left(\btheta\gv\alpha,H\right)$, whereas marginalizing out
$\btheta$ results in $\nDPM\left(\bvarphi\vert\alpha,v,\eta,S\right)$.\end{thm}
\begin{proof}
We sketch the main steps, Appendix \ref{proof_Theorem4} provides
more detail. Let $H^{*}=H_{1}\times H_{2}$, we note that when either
$H_{1}$ or $H_{2}$ are random, a result similar to Proposition \ref{Proof_Prop2}
still holds by taking the expectation on both sides of the equality.
Now let $H_{1}=H$ and $H_{2}=\DP\left(vQ_{0}\right)$ where $Q_{0}\sim\DP(\eta S)$
yields the proof for the marginalization of $\bvarphi$; let $H_{1}=\DP\left(vQ_{0}\right)$
and $H_{2}=H$ yields the proof for the marginalization of $\btheta$.
\end{proof}


